Simulations of common envelope evolution in triple systems: Circumstellar case

The dynamical evolution of triple stellar systems could induce the formation of compact binaries and binary mergers. Common envelope (CE) evolution, which plays a major role in the evolution of compact binary systems, can similarly play a key role in the evolution of triples. Here we use hydrodynamical simulations coupled with few-body dynamics to provide the first detailed models of triple common envelope (TCE) evolution. We focus on the circumstellar case, where the envelope of an evolved giant engulfs a compact binary orbiting the giant, which then in-spirals into the core of the evolved star. Through our exploratory modeling we find several possible outcomes of such TCE: (1) The merger of the binary inside the third star's envelope; (2) The disruption of the in-spiraling binary following its plunge, leading to a chaotic triple dynamics of the stellar-core and the two components of the former disrupted binary. The chaotic evolution typically leads to the in-spiral and merger of at least one of the former binary components with the core, and sometimes to the ejection of the second, or alternatively its further now-binary common-envelope evolution. The in-spiral in TCE leads to overall slower in-spiral, larger mass ejection and the production of more aspherical remnant, compared with a corresponding binary case of similar masses, due to the energy/momentum extraction from the inner-binary. We expect TCE to play a key role in producing various types of stellar-mergers and unique compact binary systems, and potentially induce transient electromagnetic and gravitational-wave sources.

==> results.tex <==
\begin{table*}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline 
 No & Masses   &$a_{\text{out}}$& Inclination & $a_{\text{in}}$ & Orbital& Outcome
\\ &(${\rm M_{\odot}}$)&(${\rm R_{\odot})}$ &&(${\rm R_{\odot})}$& phase&(merger / disruption)\tabularnewline
\hline 
\hline 
1&8 + 1 + 1 &$216$& $5^{\circ}$ & $26$ & $0^{\circ}$&core merger\tabularnewline
2&8 + 1 + 1 &$216$& $5^{\circ}$ & $3$& $0^{\circ}$&inner binary merger\tabularnewline
3&8 + 1 + 1 &$216$& $45^{\circ}$ & $26$ & $0^{\circ}$&core merger\tabularnewline
4&8 + 1 + 1 &$216$& $45^{\circ}$ & $3$ & $0^{\circ}$&inner binary merger\tabularnewline
5&8 + 1 + 1 &$216$& $5^{\circ}$ & $26$ & $90^{\circ}$&core merger\tabularnewline
6&8 + 1 + 1 &$216$& $45^{\circ}$ & $26$& $90^{\circ}$&core merger\tabularnewline
7&8 + 1 + 1 &$130$& $5^{\circ}$ & $26$ & $90^{\circ}$&core merger\tabularnewline
8&8 + 1 + 1 &$130$& $45^{\circ}$ & $26$& $90^{\circ}$&core merger\tabularnewline
9&8 + 1 + 1 &$130$& $5^{\circ}$ & $3$& $90^{\circ}$&inner binary merger\tabularnewline
10&8 + 1 + 1 &$130$& $45^{\circ}$ & $3$& $90^{\circ}$&inner binary merger\tabularnewline

11&2 + 0.6 + 0.4 & $60$ & $0^{\circ}$ & $3$ &$0^{\circ}$& inner ejection\tabularnewline
12&2 + 0.6 + 0.4 & $60$ & $0^{\circ}$ &  $13$ &$0^{\circ}$&$0.6 M_\odot $ ejection\tabularnewline
13&2 + 0.6 + 0.4 & $60$ & $0^{\circ}$ & $26$ &$0^{\circ}$&$0.4 M_\odot $ ejection\tabularnewline


14&8 + 2 & $216$ &  \multicolumn{3}{|c|}{binary common envelope}  &core merger\tabularnewline
15&2 + 1 & $60$ & \multicolumn{3}{|c|}{binary common envelope} & close stable orbit \tabularnewline
16&1 + 0.6 & $83$ & \multicolumn{3}{|c|}{binary common envelope} & close stable orbit \tabularnewline
\hline 
\end{tabular}\caption{\label{resultsummary}}
\end{table*}
